The groupoidal analogue Theta~ to Joyal's category Theta is a test category

We introduce the groupoidal analogue \tilde\Theta to Joyal's cell category \Theta and we prove that \tilde\Theta is a strict test category in the sense of Grothendieck. This implies that presheaves on \tilde\Theta model homotopy types in a canonical way. We also prove that the canonical functor from \Theta to \tilde\Theta is aspherical, again in the sense of Grothendieck. This allows us to compare weak equivalences of presheaves on \tilde\Theta to weak equivalences of presheaves on \Theta. Our proofs apply to other categories analogous to \Theta.

==> macros.tex <==
\usepackage{xspace}

\makeatletter

%
\newcommand\DeclareMathOperatorRm[1]{%
  \expandafter\DeclareMathOperator\csname #1\endcsname{#1}}

\newcommand\DeclareMathOperatorSf[1]{%
  \expandafter\DeclareMathOperator\csname #1\endcsname{\mathsf{#1}}}


% présentation
\newcommand\ndef[1]{\emph{#1}}

\def\xpoint{\futurelet\@let@token\@xpoint}
\def\@xpoint{%
  \ifx\@let@token.\else
    .%
  \fi
  \xspace}

\newcommand\zbox[1]{\makebox[0pt][l]{#1}}
\newcommand\pbox[1]{\zbox{\quad#1}}

\newcommand{\forlang}[1]{\emph{#1}}
\newcommand\ie{\forlang{i.e}\xpoint}
\newcommand{\opcit}{\forlang{op. cit}\xpoint}
\newcommand{\loccit}{loc.~cit\xpoint}



% algèbre
\DeclareMathOperator{\Coker}{Coker}

% théorie catégorie
\newcommand\C{\mathcal{C}}
\newcommand{\oo}{$\infty$\nobreakdash}
\newcommand\op{\mathrm{o}}
\newcommand\W{{\mathcal{W}}}
\newcommand\pref[1]{\widehat{#1}}
\DeclareMathOperatorSf{Ob}
\DeclareMathOperatorSf{Fl}
\DeclareMathOperatorSf{Hom}
%\DeclareMathOperatorSf{Ho}
\DeclareMathOperatorRm{Aut}
\newcommand\id[1]{{1^{}_{#1}}}

\DeclareMathOperator{\Homi}{\underline{\mathsf{Hom}}}
\DeclareMathOperator{\Homgr}{\underline{\mathsf{Hom}}_{\mathrm{\,gr}}}
\DeclareMathOperator{\Homcat}{\underline{\mathsf{Hom}}_{\mathrm{\,cat}}}
\DeclareMathOperator{\Homgl}{\underline{\mathsf{Hom}}_{\mathrm{\,gl}}}

% nom de catégories
\newcommand\Set{{\mathcal{S} \mspace{-2.mu}{et}}}
\newcommand{\Hot}{\mathsf{Hot}}
\newcommand{\Ho}[1]{\mathsf{Hot}_{#1}}

\newcommand{\@Cat}[3]{{\operatorname{\text{$#1$}\mathcal{#2C} \mspace{-2.mu}{at#3}}}}
\newcommand{\cat}{{\@Cat{}{}{}}}
\newcommand\Cat\cat
\newcommand{\ncat}[1]{{\@Cat{#1-}{}{}}}
\newcommand{\wcat}{{\@Cat{\infty-}{}{}}}

\newcommand{\@Grp}[3]{{%
  \operatorname{\text{$#1$}{\mathcal{#2G}\mspace{-0.5mu}rp\mspace{-0.01mu}d#3}}}}
\newcommand{\grp}{{\@Grp{}{}{}}}
\newcommand{\ngrp}[1]{{\@Grp{#1-}{}{}}}
\newcommand{\wgrp}{{\@Grp{\infty-}{}{}}}

\newcommand{\G}{\mathbb{G}}
\newcommand{\Gn}[1]{\mathbb{G}_{#1}}

\newcommand{\Thz}{\Theta_0}
\newcommand{\Th}{\Theta}
\newcommand{\Thtld}{\widetilde{\Theta}}

\newcommand\Mod[1]{{\operatorname{\mathrm{Mod}}(#1)}}

% axiomes
\newcommand\Ass[2]{(\mathrm{Ass}_{{#1},{#2}})}
\newcommand\Assx{(\mathrm{Ass})}
\newcommand\Exc[3]{(\mathrm{Exc}_{{#1},{#2},{#3}})}
\newcommand\Excx{(\mathrm{Exc})}
\newcommand\Lun[2]{(\mathrm{LUnit}_{{#1},{#2}})}
\newcommand\Lunx{(\mathrm{LUnit})}
\newcommand\Run[2]{(\mathrm{RUnit}_{{#1},{#2}})}
\newcommand\Runx{(\mathrm{RUnit})}
\newcommand\Fun[2]{(\mathrm{FUnit}_{{#1},{#2}})}
\newcommand\Funx{(\mathrm{FUnit})}
\newcommand\LInv[2]{(\mathrm{LInv}_{{#1},{#2}})}
\newcommand\LInvx{(\mathrm{LInv})}
\newcommand\RInv[2]{(\mathrm{RInv}_{{#1},{#2}})}
\newcommand\RInvx{(\mathrm{RInv})}
\newcommand\FInv[3]{(\mathrm{FInv}_{{#1},{#2},{#3}})}
\newcommand\FInvx{(\mathrm{FInv})}

% décalage
\newcommand\DThtld{\mathcal{D}_{\Thtld}}
\newcommand\DTh{\mathcal{D}_{\Th}}

% tableaux des dimensions
\newcommand\tabdimi[1][n]{%
{\left(
\begin{matrix}
i_1 && i_2 && \cdots && i_{#1} \cr
& i'_1 && i'_2 & \cdots & i'_{{#1}-1}
\end{matrix}
\right)}}
\newcommand\tabdimj[1][n]{%
{\left(
\begin{matrix}
j_1 && j_2 && \cdots && j_{#1} \cr
& j'_1 && j'_2 & \cdots & j'_{{#1}-1}
\end{matrix}
\right)}}
\newcommand\tabdim{{\tabdimi{}}}
\newcommand\tabdimijk{%
\left(
\begin{smallmatrix}
i & & j \cr
& k
\end{smallmatrix}
\right)}

%
\newcommand\at{\widetilde{a}}
\newcommand\Ft{\widetilde{F}}

% objets de Theta
\newcommand{\Dn}[1]{{\mathrm{D}_{#1}}}
\newcommand{\Dnt}[1]{{\widetilde{\mathrm{D}}_{#1}}}

\newcommand{\amalgd}[1]{\amalg^{}_{\Dn{#1}}}
\newcommand{\amalgdt}[1]{\amalg^{}_{\Dnt{#1}}}
\newcommand{\amalgX}[1]{\amalg^{}_{#1}}

\newcommand\Xt[1]{{\widetilde{X}_{#1}}}
\newcommand\fibrx[1]{\times^{}_{X_{#1}}}
\newcommand\fibrxt[1]{\times^{}_{\Xt{#1}}}

\newcommand\xb{\overline{x}}
\newcommand\yb{\overline{y}}
\newcommand\zb{\overline{z}}
\newcommand\tb{\overline{t}}

% morphismes de Theta
\newcommand{\Tht}[2][\@empty]{%
\ifx\@empty#1
\tau_{#2}^{}%
\else
\tau_{#1}^{#2}%
\fi
}
\newcommand{\Thtt}[2][\@empty]{%
\ifx\@empty#1
\widetilde{\tau}_{#2}^{}%
\else
\widetilde{\tau}_{#1}^{#2}%
\fi
}
\newcommand{\ThtT}[2][\@empty]{\Tht[#1]{#2}}
\newcommand{\Ths}[2][\@empty]{%
\ifx\@empty#1
\sigma_{#2}^{}%
\else
\sigma_{#1}^{#2}%
\fi
}
\newcommand{\Thst}[2][\@empty]{%
\ifx\@empty#1
\widetilde{\sigma}_{#2}^{}%
\else
\widetilde{\sigma}_{#1}^{#2}%
\fi
}
\newcommand{\ThsT}[2][\@empty]{\Ths[#1]{#2}}
\newcommand{\Thkp}[2][\@empty]{%
\ifx\@empty#1
\kappa'_{#2}%
\else
\kappa_{#1}^{'#2}%
\fi
}
\newcommand{\Thk}[2][\@empty]{%
\ifx\@empty#1
\kappa_{#2}^{}%
\else
\kappa_{#1}^{#2}%
\fi
}
\newcommand{\Thkt}[2][\@empty]{%
\ifx\@empty#1
\widetilde{\kappa}_{#2}^{}%
\else
\widetilde{\kappa}_{#1}^{#2}%
\fi
}
\newcommand{\Thnp}[2][\@empty]{%
\ifx\@empty#1
\nabla'_{#2}%
\else
\nabla_{#1}^{'#2}%
\fi
}
\newcommand{\Thn}[2][\@empty]{%
\ifx\@empty#1
\nabla_{#2}^{}%
\else
\nabla_{#1}^{#2}%
\fi
}
\newcommand{\Thnt}[2][\@empty]{%
\ifx\@empty#1
\widetilde{\nabla}_{#2}^{}%
\else
\widetilde{\nabla}_{#1}^{#2}%
\fi
}
\newcommand{\Thw}[2][\@empty]{%
\ifx\@empty#1
\Omega_{#2}^{}%
\else
\Omega_{#1}^{#2}%
\fi
}
\newcommand{\Thwt}[2][\@empty]{%
\ifx\@empty#1
\widetilde{\Omega}_{#2}^{}%
\else
\widetilde{\Omega}_{#1}^{#2}%
\fi
}

% morphisme source et but d'un ensemble globulaire
\newcommand\comp\ast
\newcommand\compt{\widetilde{\ast}\mspace{1mu}}
\newcommand\Glnto[2][\@empty]{%
\ifx\@empty#1
\widetilde{\ast}\mspace{1mu}_{#2}%
\else
    \widetilde{\ast}\mspace{1mu}_{#1}^{#2}%
  \fi
}
\newcommand\Glnt[2][\@empty]{%
  \ifx\@empty#1
    \,\widetilde{\ast}\mspace{1mu}_{#2}\,%
  \else
    \,\widetilde{\ast}\mspace{1mu}_{#1}^{#2}\,%
  \fi
}

\newcommand\Glp[1]{p^{}_{#1}}
\newcommand\Glpg[1]{pi^{}_{#1}}

\newcommand{\Glt}[2][\@empty]{%
  \ifx\@empty#1
    t_{#2}%
  \else
    t_{#1}^{#2}%
  \fi
}
\newcommand{\Gls}[2][\@empty]{%
  \ifx\@empty#1
    s_{#2}%
  \else
    s_{#1}^{#2}%
  \fi
}
\newcommand{\Gltt}[2][\@empty]{%
  \ifx\@empty#1
    \widetilde{t}_{#2}%
  \else
    \tilde{t}_{#1}^{#2}%
  \fi
}
\newcommand{\Glst}[2][\@empty]{%
  \ifx\@empty#1
    \widetilde{s}_{#2}%
  \else
    \tilde{s}_{#1}^{#2}%
  \fi
}
\newcommand{\Glw}[2][\@empty]{%
  \ifx\@empty#1
    w_{#2}^{}%
  \else
    w_{#1}^{#2}%
  \fi
}
\newcommand{\Glwt}[2][\@empty]{%
  \ifx\@empty#1
    \widetilde{w}\mspace{1mu}_{#2}^{}%
  \else
    \widetilde{w}\mspace{1mu}_{#1}^{#2}%
  \fi
}
\newcommand{\Glk}[2][\@empty]{%
  \ifx\@empty#1
    k_{#2}%
  \else
    k_{#1}^{#2}%
  \fi
}
\newcommand{\Glkt}[2][\@empty]{%
  \ifx\@empty#1
    \widetilde{k}_{#2}%
  \else
    \widetilde{k}_{#1}^{#2}%
  \fi
}
\newcommand{\Glkp}[2][\@empty]{%
  \ifx\@empty#1
    k'_{#2}%
  \else
    k_{#1}^{'#2}%
  \fi
}

% preuve Thtld
\newcommand\canu{\iota^{}_1}
\newcommand\cand{\iota^{}_2}

\renewcommand\epsilon\varepsilon

\newcommand\cepsu{{\epsilon^{}_1}}
\newcommand\cepsd{{\epsilon^{}_2}}
\newcommand\ceps[1]{{\epsilon^{}_{#1}}}
\newcommand\cepsp[1]{{\epsilon'_{#1}}}
\newcommand\cepsg[1]{\ceps{#1}}
\newcommand{\cepsi}[2]{{\epsilon^{#1}_{#2}}}
\newcommand{\cepsij}[3]{{\epsilon^{#1,#2}_{#3}}}
\newcommand{\cepsijk}[4]{%
  {\epsilon^{{#1}\, {}^{}_{\scriptstyle #2}\, #3}_{#4}}}

\makeatother

